Trust in Generative AI among students: An Exploratory Study

Generative artificial systems (GenAI) have experienced exponential growth in the past couple of years. These systems offer exciting capabilities, such as generating programs, that students can well utilize for their learning. Among many dimensions that might affect the effective adoption of GenAI, in this paper, we investigate students' \textit{trust}. Trust in GenAI influences the extent to which students adopt GenAI, in turn affecting their learning. In this study, we surveyed 253 students at two large universities to understand how much they trust \genai tools and their feedback on how GenAI impacts their performance in CS courses. Our results show that students have different levels of trust in GenAI. We also observe different levels of confidence and motivation, highlighting the need for further understanding of factors impacting trust.

==> abstract.tex <==

Generative Artificial Intelligence (\genai) systems have experienced exponential growth in the last couple of years. These systems offer exciting capabilities for CS Education (CSEd), such as generating programs, that students can well utilize for their learning.
Among the many dimensions that might affect the effective adoption of \genai for CSEd, in this paper, we investigate students' \textit{trust}. Trust in \aigen influences the extent to which students adopt \genai, in turn affecting their learning. In this paper, we present results from a survey of 253 students at two large universities to understand how much they trust \genai tools and their feedback on how \genai impacts their performance in CS courses.
Our results show that students have different levels of trust in \genai. We also observe different levels of confidence and motivation, highlighting the need for further understanding of factors impacting trust. 


==> figures/tables/experience_perception.tex <==
\begin{table*}
    \centering
    \caption{
        \label{tab:perception}
        Students self perceptions of their programming abilities based on the use of AI.
    }
    {\small \begin{tabular}%
        {
            >{\raggedright\arraybackslash}p{7.3cm}%
            >{\raggedright\arraybackslash}p{8.7cm}%
        }
        \toprule
        \multicolumn{2}{c}{ \bf Perception Distributions } \\
        {\bf Question ID} &
        \multicolumn{1}{r}{\bf Distributions}\\
        \midrule

        \bottomrule
    \end{tabular}}
\end{table*}


==> figures/tables/hackathon.tex <==
\begin{table*}
    \centering
    \caption{
        \label{tab:hackathon}
        Results
    }
    {\small \begin{tabular}{lrrrrrp{7.7cm}}
        \toprule
        & \multicolumn{3}{c}{\bf Mean Score (Rank)} \\
        \cmidrule{2-5}
        & \multicolumn{2}{c}{\bf UH}
        & \multicolumn{2}{c}{\bf IITK} \\
        \cmidrule{2-5}
        {\bf Question ID} &
        {\bf Users} &
        {\bf Heard} &
        {\bf User} &
        {\bf Heard} &
        \multicolumn{2}{r}{\bf Distribution (All)}\\
        \midrule
        \multicolumn{5}{c}{ \bf Trust } &
        \multicolumn{2}{r}{\legendbox{30} Strong Disagree \, \legendbox{60} Disagree \, \legendbox{90} Neutral \, \legendbox{120} Agree \, \legendbox{150} Strong Agree} \\
        \midrule
            \input figures/tables/data/trust
        \midrule
        \multicolumn{5}{c}{ \bf Perceptions } &
        \multicolumn{2}{r}{\legendbox{30} Strong Disagree \, \legendbox{60} Disagree \, \legendbox{90} Neutral \, \legendbox{120} Agree \, \legendbox{150} Strong Agree} \\
        \midrule
            \input figures/tables/data/trust
        \midrule
        \multicolumn{5}{c}{ \bf Usage } &
        \multicolumn{2}{r}{\legendbox{30} Strong Disagree \, \legendbox{60} Disagree \, \legendbox{90} Neutral \, \legendbox{120} Agree \, \legendbox{150} Strong Agree} \\
        \midrule
            \input figures/tables/data/trust
        \bottomrule
    \end{tabular}}
\end{table*}


==> figures/tables/perception.tex <==
\begin{table*}
    \centering
    \caption{
        \label{tab:perception}
        Students self perceptions of their programming abilities based on the use of AI.
    }
    {\small \begin{tabular}%
        {
            >{\raggedright\arraybackslash}p{6.4cm}%
            >{\raggedleft\arraybackslash}p{0.8cm}%
            >{\raggedleft\arraybackslash}p{8.7cm}%
        }
        \toprule
        \multicolumn{2}{c}{ \bf Perception Distributions } \\
        {\bf Question ID} &
        \multicolumn{1}{r}{\bf Distributions}\\
        \midrule
        \multicolumn{1}{l}{ \bf Confidence All } &
        { \bf Count } &
        \multicolumn{1}{r}{
            \legendbox{100}{Firebrick1} Strong Disagree \,
            \legendbox{50}{Firebrick1} Disagree \,
            \legendbox{30}{gray} Neutral \,
            \legendbox{30}{Green1} Agree \,
            \legendbox{100}{Green1} Strong Agree
        } \\
        \midrule
            \input figures/tables/data/confidence \\

        \multicolumn{1}{l}{ \bf Confidence Gender } &
        { \bf Count } &
        \multicolumn{1}{r}{
            \legendbox{100}{Firebrick1} Strong Disagree \,
            \legendbox{50}{Firebrick1} Disagree \,
            \legendbox{30}{gray} Neutral \,
            \legendbox{30}{Green1} Agree \,
            \legendbox{100}{Green1} Strong Agree
        } \\
        \midrule
            \input figures/tables/data/gender_confidence \\

        \multicolumn{1}{l}{ \bf Confidence if they use AI tools } &
        { \bf Count } &
        \multicolumn{1}{r}{
            \legendbox{100}{Firebrick1} Strong Disagree \,
            \legendbox{50}{Firebrick1} Disagree \,
            \legendbox{30}{gray} Neutral \,
            \legendbox{30}{Green1} Agree \,
            \legendbox{100}{Green1} Strong Agree
        } \\
        \midrule
            \input figures/tables/data/use_ai_confidence \\

        \bottomrule
    \end{tabular}}
\end{table*}


==> figures/tables/perception2.tex <==

\begin{table*}
    \centering
    \caption{
        \label{tab:perceptiontwo}
        Students self perceptions of their programming abilities based on the use of AI.
    }
    {\small \begin{tabular}%
        {
            >{\raggedright\arraybackslash}p{6.4cm}%
            >{\raggedleft\arraybackslash}p{0.8cm}%
            >{\raggedleft\arraybackslash}p{8.7cm}%
        }
        \toprule
        \multicolumn{3}{c}{ \bf Perception Distributions } \\
        {\bf Question ID} &
        \multicolumn{2}{r}{\bf Distributions}\\
        \midrule

        \multicolumn{1}{l}{ \bf Confidence Helpful AI } \legendbox{100}{white}- \legendbox{20}{gray}Neutral \legendbox{60}{LightBlue1}+ &
        { \bf Count } &
        \multicolumn{1}{r}{
            \legendbox{100}{Firebrick1} Strong Disagree \,
            \legendbox{50}{Firebrick1} Disagree \,
            \legendbox{30}{gray} Neutral \,
            \legendbox{30}{Green1} Agree \,
            \legendbox{100}{Green1} Strong Agree
        } \\
        \midrule
            \input figures/tables/data/helpfulness_confidence \\

        \multicolumn{1}{l}{ \bf Confidence FirstGen } &
        { \bf Count } &
        \multicolumn{1}{r}{
            \legendbox{100}{Firebrick1} Strong Disagree \,
            \legendbox{50}{Firebrick1} Disagree \,
            \legendbox{30}{gray} Neutral \,
            \legendbox{30}{Green1} Agree \,
            \legendbox{100}{Green1} Strong Agree
        } \\
        \midrule
            \input figures/tables/data/generation_confidence \\

        \multicolumn{1}{l}{ \bf Confidence Location } &
        { \bf Count } &
        \multicolumn{1}{r}{
            \legendbox{100}{Firebrick1} Strong Disagree \,
            \legendbox{50}{Firebrick1} Disagree \,
            \legendbox{30}{gray} Neutral \,
            \legendbox{30}{Green1} Agree \,
            \legendbox{100}{Green1} Strong Agree
        } \\
        \midrule
            \input figures/tables/data/location_confidence \\

        \bottomrule
    \end{tabular}}
\end{table*}


==> sections/quant/rq3.tex <==
\subsection{How do students perceive their own programming abilities, given their use of AI (or not)?}

% \subsubsection{Quant}

\textbf{Include distribution chart showing this data.}

% Distributions for AI vs. NonAI of the response for the following questions:

% \begin{list}{}{\leftmargin=1em}
%     \item \textbf{1.} I feel confident completing programming assignments by myself.
%     \item \textbf{2.} I feel confident finding the steps to solve a programming assignment.
%     \item \textbf{3.} I feel confident finding ways out when I am stuck on a programming problem.
% \end{list}

\input{figures/tables/perception.tex}
%\input{figures/tables/perception2.tex}

% \textbf{Summary}
Table~\ref{tab:perception} summarizes reported students' confidence. 
Overall the responses to confidence are positive; with more than 55\% for any of the 3 questions being positive, regardless of whether they use AI or not.
In fact there does not seem to be any difference on someone's perception of their own programming abilities based on whether they use AI or not.

%\observation{There is no difference in confidence between \genai users and non-users.}

==> table_demographics_locationwise.tex <==
\begin{table}[h!]
\setlength{\arrayrulewidth}{0.1mm}
\setlength{\tabcolsep}{12pt}
\begin{tabular}{ |p{3.2cm}|r| } \hline \hline
\rowcolor{Snow3} {\textbf{Demographics}} & \IIT \\ \hline
\rowcolor{LightBlue1} \multicolumn{2}{|l|}{\textbf{Gender}} \\ \hline
    Male & 110 \\
    Female & 12 \\
    Other & 1 \\
    Prefer Not to Say & 1\\ \hline
\rowcolor{LightBlue1} \multicolumn{2}{|l|}{\textbf{First Generation Student}} \\ \hline
    Continuing Generation & 92 \\ 
    First Generation & 32 \\ \hline
\rowcolor{LightBlue1} \multicolumn{2}{|l|}{\textbf{Major}} \\ \hline
    Computer Science & 33 \\
    Other Engineering & 59 \\
    Science/Medicine & 17 \\
    Other & 13 \\
    Arts/Humanities & 2 \\ \hline
\rowcolor{LightBlue1} \multicolumn{2}{|l|}{\textbf{AI Users}} \\ \hline
    User & 115 \\
    Non-User & 9 \\ \hline \hline
\end{tabular}
\caption{The table provides an overview of the demographics for \IIT participants}
\label{tbl:DEMOIITK} 
\end{table}

\begin{table}[h!]
    \setlength{\arrayrulewidth}{0.1mm}
    \setlength{\tabcolsep}{12pt}
    \begin{tabular}{ |p{3.2cm}|r| } \hline \hline
    \rowcolor{Snow3} {\textbf{Demographics}} & \UH \\ \hline
    \rowcolor{LightBlue1} \multicolumn{2}{|l|}{\textbf{Gender}} \\ \hline
        Male & 100 \\
        Female & 27 \\
        Other & 1 \\
        Prefer Not to Say & 1\\ \hline
    \rowcolor{LightBlue1} \multicolumn{2}{|l|}{\textbf{First Generation Student}} \\ \hline
        Continuing Generation & 70 \\ 
        First Generation & 59 \\ \hline
    \rowcolor{LightBlue1} \multicolumn{2}{|l|}{\textbf{Major}} \\ \hline
        Computer Science & 120 \\
        Other Engineering & 4 \\
        Science/Medicine & 2 \\
        Other & 1 \\
        Arts/Humanities & 2 \\ \hline
    \rowcolor{LightBlue1} \multicolumn{2}{|l|}{\textbf{AI Users}} \\ \hline
        User & 101 \\
        Non-User & 28 \\ \hline \hline
    \end{tabular}
    \caption{The table provides an overview of the demographics for \UH participants}
    \label{tbl:DEMOUH} 
    \end{table}
